Divide and Conquer: One-Bit MIMO-OFDM Detection by Inexact Expectation Maximization

Adopting one-bit analog-to-digital convertors (ADCs) for massive multiple-input multiple-output (MIMO) implementations has great potential in reducing the hardware cost and power consumption. However, distortions caused by quantization raise great challenges. In MIMO orthogonal frequency-division modulation (OFDM) detection, coarse quantization renders the orthogonal separation among subcarriers inapplicable, forcing us to deal with a problem that has a very large problem size. In this paper we study the expectation-maximization (EM) approach for one-bit MIMO-OFDM detection. The idea is to iteratively decouple the MIMO-OFDM detection problem among subcarriers. Using the perspective of block coordinate descent, we describe inexact variants of the classical EM method for providing more flexible and computationally efficient designs. Simulation results are provided to illustrate the potential of the divide-and-conquer strategy enabled by EM.

==> sym_marco.tex <==
%make sure to keep this for convenience later
\newcommand\bw{\ensuremath{{\bm w}}}
\newcommand\bW{\ensuremath{{\bm W}}}
\newcommand\cW{\ensuremath{\bm{\mathcal{W}}}}
\newcommand\bbw{\ensuremath{{\bar{\bm w}}}}
\newcommand\bq{\ensuremath{{\bm q}}}
\newcommand\bx{\ensuremath{{\bm x}}}
\newcommand\by{\ensuremath{{\bm y}}}
\newcommand\bG{\ensuremath{{\bm G}}}
\newcommand\bh{\ensuremath{{\bm h}}}
\newcommand\bH{\ensuremath{{\bm H}}}
\newcommand\cH{\ensuremath{\bm{\mathcal{H}}}}
\newcommand\bbh{\ensuremath{\bar{\bm h}}}
\newcommand\hbh{\ensuremath{\hat{\bm h}}}
\newcommand\be{\ensuremath{{\bm e}}}
\newcommand\bz{\ensuremath{{\bm z}}}
\newcommand\bp{\ensuremath{{\bm p}}}
\newcommand\bP{\ensuremath{{\bm P}}}
\newcommand\bR{\ensuremath{{\bm R}}}
\newcommand\bT{\ensuremath{{\bm T}}}
\newcommand\bX{\ensuremath{{\bm X}}}
\newcommand\bZ{\ensuremath{{\bm Z}}}
\newcommand\cZ{\ensuremath{\bm{\mathcal{Z}}}}
\newcommand\bC{\ensuremath{{\bm C}}}
\newcommand\bc{\ensuremath{{\bm c}}}
\newcommand\ba{\ensuremath{{\bm a}}}
\newcommand\bba{\ensuremath{\bar{\bm a}}}
\newcommand\bA{\ensuremath{{\bm A}}}
\newcommand\bbA{\ensuremath{\bar{\bm A}}}
\newcommand\bb{\ensuremath{{\bm b}}}
\newcommand\bg{\ensuremath{{\bm g}}}
\newcommand\bB{\ensuremath{{\bm B}}}
\newcommand\blam{\ensuremath{{\bm \lambda}}}
\newcommand\bmu{\ensuremath{{\bm \mu}}}
\newcommand\balp{\ensuremath{{\bm \alpha}}}
\newcommand\bbeta{\ensuremath{{\bm \beta}}}
\newcommand\bXi{\ensuremath{{\bm \Xi}}}
\newcommand\bPi{\ensuremath{{\bm \Pi}}}
\newcommand\bbPi{\ensuremath{\bar{\bm \Pi}}}
\newcommand\bF{\ensuremath{{\bm F}}}
\newcommand\bbF{\ensuremath{\bar{\bm F}}}
\newcommand\bd{\ensuremath{{\bm d}}}
\newcommand\bD{\ensuremath{{\bm D}}}
\newcommand\bu{\ensuremath{{\bm u}}}
\newcommand\bv{\ensuremath{{\bm v}}}
\newcommand\bSig{\ensuremath{{\bm \Sigma}}}
\newcommand\bsig{\ensuremath{{\bm \sigma}}}
\newcommand\beeta{\ensuremath{{\bm \eta}}}
\newcommand\bPhi{\ensuremath{{\bm \Phi}}}
\newcommand\bPsi{\ensuremath{{\bm \Psi}}}
\newcommand\btheta{\ensuremath{{\bm \theta}}}
\newcommand\bTheta{\ensuremath{{\bm \Theta}}}
\newcommand\bomega{\ensuremath{{\bm \omega}}}
\newcommand\bxi{\ensuremath{{\bm \xi}}}
\newcommand\bzeta{\ensuremath{{\bm \zeta}}}

\newcommand\bYh{\ensuremath{{\bm Y}_{\rm H}}}
\newcommand\bYm{\ensuremath{{\bm Y}_{\rm M}}}
\newcommand\byh{\ensuremath{{\bm y}_{\rm H}}}
\newcommand\bym{\ensuremath{{\bm y}_{\rm M}}}
\newcommand\bAm{\ensuremath{{\bm A}_{\rm M}}}
\newcommand\bDh{\ensuremath{{\bm D}_{\rm H}}}
\newcommand\bDm{\ensuremath{{\bm D}_{\rm M}}}
\newcommand\bDx{\ensuremath{{\bm D}_{\rm X}}}
\newcommand\bVh{\ensuremath{{\bm V}_{\rm H}}}
\newcommand\bVm{\ensuremath{{\bm V}_{\rm M}}}
\newcommand\Lh{\ensuremath{L_{\rm H}}}
\newcommand\Mm{\ensuremath{M_{\rm M}}}


\newcommand\bY{\ensuremath{{\bm Y}}}
\newcommand\bV{\ensuremath{{\bm V}}}
\newcommand\bU{\ensuremath{{\bm U}}}
\newcommand\bs{\ensuremath{{\bm s}}}
\newcommand\bS{\ensuremath{{\bm S}}}
\newcommand\bE{\ensuremath{{\bm E}}}

\newcommand{\Rbb}{\mathbb{R}}
\newcommand{\Cbb}{\mathbb{C}}
\newcommand{\Hbb}{\mathbb{H}}
\newcommand{\Sbb}{\mathbb{S}}

\newcommand{\setA}{\mathcal{A}}
\newcommand{\setB}{\mathcal{B}}
\newcommand{\setD}{\mathcal{D}}
\newcommand{\setH}{\mathcal{H}}
\newcommand{\setX}{\mathcal{X}}
\newcommand{\setR}{\mathcal{R}}
\newcommand{\setU}{\mathcal{U}}
\newcommand{\setV}{\mathcal{V}}
\newcommand{\setS}{\mathcal{S}}
\newcommand{\setC}{\mathcal{C}}
\newcommand{\setN}{\mathcal{N}}
\newcommand{\setL}{\mathcal{L}}

\newcommand{\N}{\mathcal{N}}
\newcommand{\CN}{\mathcal{CN}}
\newcommand{\Exp}{\mathbb{E}}
\newcommand{\jj}{\mathfrak{j}}
\newcommand{\dec}{\mathrm{dec}}
\newcommand{\Diag}{\mathrm{Diag}}
\newcommand{\diag}{\mathrm{diag}}

\newcommand\bQ{\ensuremath{{\bm Q}}}
\newcommand\bLam{\ensuremath{{\bm \Lambda}}}
\newcommand\br{\ensuremath{{\bm r}}}

\newcommand\Ree{\ensuremath{{\rm Re}}}
\newcommand\Imm{\ensuremath{{\rm Im}}}
\newcommand{\eps}{\varepsilon}
\newcommand{\bzero}{{\bm 0}}
\newcommand{\bone}{{\bm 1}}
\newcommand{\bI}{{\bm I}}
\newcommand*{\LargerCdot}{\raisebox{-0.25ex}{\scalebox{1.2}{$\cdot$}}}
\newcommand\vvec{\ensuremath{{\rm vec}}}
\newcommand\mmat{\ensuremath{{\rm mat}}}
\newcommand\bigO{\ensuremath{{\mathcal{O}}}}

\newcommand{\lammax}{\lambda_{\rm max}}
\newcommand{\lammin}{\lambda_{\rm min}}
\newcommand{\betamaxi}{\beta^{\sf max}_i}
\newcommand{\betamini}{\beta^{\sf min}_i}
%\newcommand{\hbetamini}{\hat{\beta}^{\sf min}_i}
\newcommand{\hbetamini}{{\delta_i}}
%\newcommand\hbetamin[1]{\hat{\beta}^{\sf min}_{#1}}
\newcommand\hbetamin[1]{{\delta_{#1}}}
\newcommand{\hbetainiti}{\hat{\beta}^{\sf init}_i}

%\newcommand{\hbetai}{{\green \hat{\beta}_i(\bx_{-i})}}
\newcommand{\hbetai}{{\hat{\beta}_i}}
\newcommand{\hRi}{{\hat{\bR}_i}}

\newcommand{\aalp}{{\alpha_i}}
\newcommand\aaalp[1]{{\alpha_{#1}}}
\newcommand{\setI}{\mathcal{I}}

\newcommand\indfn[1]{{{\mathbbm 1}_{#1}}}
%\newcommand\indfn{\ensuremath{{\mathbbm 1}}}
\newcommand\prox{\ensuremath{{\sf prox}}}
\newcommand\LO{\ensuremath{{\sf LO}}}

\newcommand\update{\ensuremath{{\sf UD}}}
\newcommand\bxex{\ensuremath{{\bm x}_{\rm ex}}}
\newcommand\bxkil{\bm x^{k,i,\ell}}
\newcommand\bxki[1]{\bm x^{k,i,#1}}
\newcommand\bxk[2]{\bm x^{k,#1,#2}}
\newcommand\dF[1]{\Delta_{#1}}
\newcommand\dx[1]{e_{#1}}
\newcommand\tdx[1]{\tilde{e}_{#1}}

\newcommand\A[1]{{\sf A#1)}}

\newcommand\sspan{\ensuremath{{\rm span}}}
\newcommand\aff{\ensuremath{{\rm aff}}}
\newcommand\conv{\ensuremath{{\rm conv}}}
\newcommand\bconv{\ensuremath{\overline{\rm conv}}}
\newcommand\var{\ensuremath{{\rm var}}}
\newcommand\cov{\ensuremath{{\rm Cov}}}
\newcommand\svol{\ensuremath{{\rm vol}}}
\newcommand\TVar{\ensuremath{{\rm tvar}}}
\newcommand\tr{\ensuremath{{\rm tr}}}



